Behavior and Sublinear Algorithm for Opinion Disagreement on Noisy Social Networks

The phenomenon of opinion disagreement has been empirically observed and reported in the literature, which is affected by various factors, such as the structure of social networks. An important discovery in network science is that most real-life networks, including social networks, are scale-free and sparse. In this paper, we study noisy opinion dynamics in sparse scale-free social networks to uncover the influence of power-law topology on opinion disagreement. We adopt the popular discrete-time DeGroot model for opinion dynamics in a graph, where nodes' opinions are subject to white noise. We first study opinion disagreement in many realistic and model networks with a scale-free topology, which approaches a constant, indicating that a scale-free structure is resistant to noise in the opinion dynamics. Moreover, existing algorithms for estimating opinion disagreement are computationally impractical for large-scale networks due to their high computational complexity. To solve this challenge, we introduce a sublinear-time algorithm to approximate this quantity with a theoretically guaranteed error. This algorithm efficiently simulates truncated random walks starting from a subset of nodes while preserving accurate estimation. Extensive experiments demonstrate its efficiency, accuracy, and scalability.

==> src/alg/approxdelta_old.tex <==
\begin{algorithm}
    \caption{\textsc{ApproxDelta}$(\calG, \epsilon)$}
    \label{alg:approx_delta}
    \Input{
        $\G(\V, \E, w) $: a connected undirected weighted graph \\
        $\epsilon$: an approximation parameter \\
    }
    \Output{
        $\tilde{\delta}$: approximation of opinion disagreement $\delta$ in $\G$
    }
    $\tilde{\G}=$ \textsc{Sparisify}$(\G,\eps)$\;
    $\bar{\G}$: graph obtained from $\tilde{\G}$ by removing self-loops \;
    $\bar{\LL}=$ Laplacian of $\bar{\G}$\;%,\, $\bar{d}_i=$ the degree of node $i$ in $\bar{\G}$, $\bar{d}_{\rm sum}=\sum_{i \in \V} \bar{d}_i$
    Construct a matrix $\QQ_{k \times \bar{M}}$, where $k=\lceil 24\log N/\epsilon^2 \rceil$ and each entry is $\pm 1/\sqrt{k}$ with identical probability\;
    \For{$i=1$ to $k$}{
        $\qq_i^\top $=the $i$-th row of $\QQ_{k \times \bar{M}} \bar{\WW}^{1/2} \bar{\BB}$ \\
        $\tilde{\zz}_i=\mathtt{LaplSolve}(\bar{\LL}, \qq_i, \kappa)$ where parameter $\kappa$ is given by~(5)\\
    }
    Calculate the constant vector ${\bf p}=\ZZtil \ppi$\;
    \For{each $i \in \V$}{
    $\tilde{C}(i)= \|\ZZtil_{:,u}-{\bf p}\|^2$
    }
    $\tilde{\delta}=d_{\rm sum}\,\sum_{i=1}^N \pi_i^2\cdot \tilde{C}(i)$\;
    \Return $\tilde{\delta}$
\end{algorithm}

==> src/header.tex <==
\usepackage{booktabs}
\usepackage[ruled]{algorithm2e}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}

\usepackage{amsmath,amssymb,amsfonts}
\usepackage{comment}
\allowdisplaybreaks
\let\Bbbk\relax
\usepackage{latexsym}
\usepackage{siunitx}
\newcommand\bmmax{2}
\usepackage{bm}
\usepackage{nicefrac}
%\usepackage[usenames]{color}
\usepackage{booktabs}
\usepackage{array}
\usepackage{multirow}
\usepackage[para,online,flushleft]{threeparttable}
\usepackage{makecell}
%\usepackage[procnumbered,ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{stfloats}
\usepackage{graphicx}
\usepackage{color}
\usepackage{url}

\usepackage{tabularx}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{siunitx}
\usepackage{subfigure}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\def\proof{{\bf Proof.}\hskip 0.3truecm}
\def\endproof{\quad $\Box$}

\allowdisplaybreaks[3]

\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
\usepackage{textcomp}
\usepackage{url}
\usepackage{verbatim}
\usepackage{cite}
\hyphenation{op-tical net-works semi-conduc-tor IEEE-Xplore}
% updated with editorial comments 8/9/2021
\hyphenation{}

% Algorithm2e
\DontPrintSemicolon
\SetKw{KwAnd}{and}
%\SetProcnameSty{textsc}
\SetFuncSty{textsc}
\SetKwInOut{Input}{Input\ \ \ \ }
\SetKwInOut{Output}{Output}

\newenvironment{envblue}{}{}

\newcommand{\smblue}[1]{{#1}}
\newcommand\ppi{\boldsymbol{\pi}}
\newcommand\ppsi{\boldsymbol{\mathit{\psi}}}
\newcommand\SSigma{\boldsymbol{\Sigma}}

\newcommand\bb{\boldsymbol{\mathit{b}}}
\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\ee{\boldsymbol{\mathit{e}}}
\newcommand\ii{\boldsymbol{\mathit{i}}}
\newcommand\qq{\boldsymbol{\mathit{q}}}
\newcommand\uu{\boldsymbol{\mathit{u}}}
%\renewcommand\vv{\boldsymbol{\mathit{v}}}
\newcommand\xx{\boldsymbol{\mathit{x}}}
\newcommand\yy{\boldsymbol{\mathit{y}}}
\newcommand\zz{\boldsymbol{\mathit{z}}}

\renewcommand\AA{\boldsymbol{\mathit{A}}}
\newcommand\BB{\boldsymbol{\mathit{B}}}
\newcommand\DD{\boldsymbol{\mathit{D}}}
\newcommand\HH{\boldsymbol{\mathit{H}}}
\newcommand\II{\boldsymbol{\mathit{I}}}
\newcommand\JJ{\boldsymbol{\mathit{J}}}
\newcommand\LL{\boldsymbol{\mathit{L}}}
\newcommand\calLL{\boldsymbol{\mathcal{L}}}
\newcommand\MM{\boldsymbol{\mathit{M}}}
\newcommand\OO{\mathbf{O}}
\newcommand\PP{\boldsymbol{\mathit{P}}}
\newcommand\QQ{\boldsymbol{\mathit{Q}}}
\newcommand\RR{\boldsymbol{\mathit{R}}}
\newcommand\XX{\boldsymbol{\mathit{X}}}
\renewcommand\SS{\boldsymbol{\mathit{S}}}
\newcommand\WW{\boldsymbol{\mathit{W}}}
\newcommand\ZZ{\boldsymbol{\mathit{Z}}}
\newcommand\YY{\boldsymbol{\mathit{Y}}}
\newcommand\YYtil{\boldsymbol{\mathit{\tilde{Y}}}}

\newcommand\Otil{\widetilde{O}}
\newcommand\ZZtil{\boldsymbol{\mathit{\tilde{Z}}}}
\newcommand\LLtil{\boldsymbol{\mathit{\tilde{L}}}}
\newcommand\LLbar{\boldsymbol{\mathit{\bar{L}}}}

\newcommand{\expec}[1]{\textbf{E} \left\{ #1 \right\} }
\newcommand{\var}[1]{\textbf{var} \left\{ #1 \right\} }
\newcommand{\tr}[1]{\textbf{tr} \left( #1 \right) }

\newcommand{\UV}[1]{\ensuremath{\mathbf{I}_{#1}}}
\newcommand{\AO}[1]{\ensuremath{\mathbf{1}_{#1}}}

\newcommand{\Lap}{\ensuremath{\mathbf{L}}}
\newcommand{\A}{\ensuremath{\mathbf{A}}}
\newcommand{\D}{\ensuremath{\mathbf{D}}}
\newcommand{\Prj}{\ensuremath{\mathbf{\Pi}}}
\newcommand{\T}{\ensuremath{\top}}
\newcommand{\Limg}{\ensuremath{\lim_{g\rightarrow\infty}}}
\newcommand{\Hso}{\ensuremath{H_{\mathrm{SO}}}}
\newcommand{\tilHso}{\ensuremath{\tilde{H}_{\mathrm{SO}}}}
\newcommand{\Hfo}{\ensuremath{H_{\mathrm{FO}}}}

\newcommand\bbeta{\boldsymbol{\beta}}
\newcommand\lamtil{\tilde{\lambda}}

\newcommand{\B}{\mathcal{B}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\N}{{\mathcal N}}
\newcommand{\F}{{\cal F}}
\newcommand{\Hh}{{\cal H}}
\newcommand{\Pp}{{\cal P}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}

\newcommand{\kh}[1]{\left(#1\right)}
\def\abs#1{\left|#1  \right|}
\def\norm#1{\left\| #1 \right\|}
\def\calG{\mathcal{G}}
\def\G{\mathcal{G}}
\def\eps{\epsilon}
\newcommand{\one}{\mathbf{1}}
\newcommand{\zero}{\mathbf{0}}
\def\trace#1{\mathrm{Tr} \left(#1 \right)}
\def\defeq{\stackrel{\mathrm{def}}{=}}

\newcommand{\mat}[1]{\boldsymbol{#1}}
%\renewcommand{\vec}[1]{\boldsymbol{\mathrm{#1}}}
%\newcommand{\vecalt}[1]{\boldsymbol{#1}}
\renewcommand{\vec}[1]{\boldsymbol{#1}}

\newcommand{\eye}{\mat{I}\xspace}
\newcommand{\mA}{\ensuremath{\mat{A}}\xspace}
\newcommand{\mB}{\ensuremath{\mat{B}}\xspace}
\newcommand{\mC}{\ensuremath{\mat{C}}\xspace}
\newcommand{\mD}{\ensuremath{\mat{D}}\xspace}
\newcommand{\mE}{\ensuremath{\mat{E}}\xspace}
\newcommand{\mF}{\ensuremath{\mat{F}}\xspace}
\newcommand{\mG}{\ensuremath{\mat{G}}\xspace}
\newcommand{\mH}{\ensuremath{\mat{H}}\xspace}
\newcommand{\mI}{\ensuremath{\mat{I}}\xspace}
\newcommand{\mJ}{\ensuremath{\mat{J}}\xspace}
\newcommand{\mK}{\ensuremath{\mat{K}}\xspace}
\newcommand{\mL}{\ensuremath{\mat{L}}\xspace}
\newcommand{\mM}{\ensuremath{\mat{M}}\xspace}
\newcommand{\mN}{\ensuremath{\mat{N}}\xspace}
\newcommand{\mO}{\ensuremath{\mat{O}}\xspace}
\newcommand{\mP}{\ensuremath{\mat{P}}\xspace}
\newcommand{\mQ}{\ensuremath{\mat{Q}}\xspace}
\newcommand{\mR}{\ensuremath{\mat{R}}\xspace}
\newcommand{\mS}{\ensuremath{\mat{S}}\xspace}
\newcommand{\mT}{\ensuremath{\mat{T}}\xspace}
\newcommand{\mU}{\ensuremath{\mat{U}}\xspace}
\newcommand{\mV}{\ensuremath{\mat{V}}\xspace}
\newcommand{\mW}{\ensuremath{\mat{W}}\xspace}
\newcommand{\mX}{\ensuremath{\mat{X}}\xspace}
\newcommand{\mY}{\ensuremath{\mat{Y}}\xspace}
\newcommand{\mZ}{\ensuremath{\mat{Z}}\xspace}
\newcommand{\mLambda}{\ensuremath{\mat{\Lambda}}\xspace}
\newcommand{\mSigma}{\ensuremath{\mat{\Sigma}}\xspace}
\newcommand{\mPbar}{\bar{\mP}\xspace}

\newcommand{\ones}{\vec{1}\xspace}
\newcommand{\va}{\ensuremath{\vec{a}}\xspace}
\newcommand{\vb}{\ensuremath{\vec{b}}\xspace}
\newcommand{\vc}{\ensuremath{\vec{c}}\xspace}
\newcommand{\vd}{\ensuremath{\vec{d}}\xspace}
\newcommand{\ve}{\ensuremath{\vec{e}}\xspace}
\newcommand{\vf}{\ensuremath{\vec{f}}\xspace}
\newcommand{\vg}{\ensuremath{\vec{g}}\xspace}
\newcommand{\vh}{\ensuremath{\vec{h}}\xspace}
\newcommand{\vi}{\ensuremath{\vec{i}}\xspace}
\newcommand{\vj}{\ensuremath{\vec{j}}\xspace}
\newcommand{\vk}{\ensuremath{\vec{k}}\xspace}
\newcommand{\vl}{\ensuremath{\vec{l}}\xspace}
\newcommand{\vm}{\ensuremath{\vec{l}}\xspace}
\newcommand{\vn}{\ensuremath{\vec{N}}\xspace}
\newcommand{\vo}{\ensuremath{\vec{o}}\xspace}
\newcommand{\vp}{\ensuremath{\vec{p}}\xspace}
\newcommand{\vq}{\ensuremath{\vec{q}}\xspace}
\newcommand{\vr}{\ensuremath{\vec{r}}\xspace}
\newcommand{\vs}{\ensuremath{\vec{s}}\xspace}
\newcommand{\vt}{\ensuremath{\vec{t}}\xspace}
\newcommand{\vu}{\ensuremath{\vec{u}}\xspace}
\newcommand{\mvv}{\ensuremath{\vec{v}}\xspace}
\newcommand{\vw}{\ensuremath{\vec{w}}\xspace}
\newcommand{\vx}{\ensuremath{\vec{x}}\xspace}
\newcommand{\vy}{\ensuremath{\vec{y}}\xspace}
\newcommand{\vz}{\ensuremath{\vec{z}}\xspace}
\newcommand{\vpi}{\ensuremath{\vecalt{\pi}}\xspace}
\newcommand{\vzero}{\ensuremath{\vec{0}}\xspace}
\newcommand{\vsigma}{\ensuremath{\vecalt{\sigma}}\xspace}
\newcommand{\valpha}{\ensuremath{\vecalt{\alpha}}\xspace}
\newcommand{\vlambda}{\ensuremath{\vecalt{\lambda}}\xspace}

%% Black-board Bold Alphabets
\newcommand{\bbA}{\ensuremath{{\mathbb A}}\xspace}
\newcommand{\bbB}{\ensuremath{{\mathbb B}}\xspace}
\newcommand{\bbC}{\ensuremath{{\mathbb C}}\xspace}
\newcommand{\bbD}{\ensuremath{{\mathbb D}}\xspace}
\newcommand{\bbE}{\ensuremath{{\mathbb E}}\xspace}
\newcommand{\bbF}{\ensuremath{{\mathbb F}}\xspace}
\newcommand{\bbG}{\ensuremath{{\mathbb G}}\xspace}
\newcommand{\bbH}{\ensuremath{{\mathbb H}}\xspace}
\newcommand{\bbI}{\ensuremath{{\mathbb I}}\xspace}
\newcommand{\bbJ}{\ensuremath{{\mathbb J}}\xspace}
\newcommand{\bbK}{\ensuremath{{\mathbb K}}\xspace}
\newcommand{\bbL}{\ensuremath{{\mathbb L}}\xspace}
\newcommand{\bbN}{\ensuremath{{\mathbb N}}\xspace}
\newcommand{\bbO}{\ensuremath{{\mathbb O}}\xspace}
\newcommand{\bbP}{\ensuremath{{\mathbb P}}\xspace}
\newcommand{\bbQ}{\ensuremath{{\mathbb Q}}\xspace}
\newcommand{\bbR}{\ensuremath{{\mathbb R}}\xspace}
\newcommand{\bbS}{\ensuremath{{\mathbb S}}\xspace}
\newcommand{\bbT}{\ensuremath{{\mathbb T}}\xspace}
\newcommand{\bbU}{\ensuremath{{\mathbb U}}\xspace}
\newcommand{\bbV}{\ensuremath{{\mathbb V}}\xspace}
\newcommand{\bbX}{\ensuremath{{\mathbb X}}\xspace}
\newcommand{\bbZ}{\ensuremath{{\mathbb Z}}\xspace}
\newcommand{\indic}{\ensuremath{{\mathbbm 1}}\xspace}

%% Cal Alphabets
\newcommand{\cA}{\ensuremath{{\mathcal A}}\xspace}
\newcommand{\cB}{\ensuremath{{\mathcal B}}\xspace}
\newcommand{\cC}{\ensuremath{{\mathcal C}}\xspace}
\newcommand{\cD}{\ensuremath{{\mathcal D}}\xspace}
\newcommand{\cE}{\ensuremath{{\mathcal E}}\xspace}
\newcommand{\cF}{\ensuremath{{\mathcal F}}\xspace}
\newcommand{\cG}{\ensuremath{{\mathcal G}}\xspace}
\newcommand{\cH}{\ensuremath{{\mathcal H}}\xspace}
\newcommand{\cI}{\ensuremath{{\mathcal I}}\xspace}
\newcommand{\cK}{\ensuremath{{\mathcal K}}\xspace}
\newcommand{\cL}{\ensuremath{{\mathcal L}}\xspace}
\newcommand{\cM}{\ensuremath{{\mathcal M}}\xspace}
\newcommand{\cN}{\ensuremath{{\mathcal N}}\xspace}
\newcommand{\cO}{\ensuremath{{\mathcal O}}\xspace}
\newcommand{\cP}{\ensuremath{{\mathcal P}}\xspace}
\newcommand{\cQ}{\ensuremath{{\mathcal Q}}\xspace}
\newcommand{\cR}{\ensuremath{{\mathcal R}}\xspace}
\newcommand{\cS}{\ensuremath{{\mathcal S}}\xspace}
\newcommand{\cT}{\ensuremath{{\mathcal T}}\xspace}
\newcommand{\cU}{\ensuremath{{\mathcal U}}\xspace}
\newcommand{\cV}{\ensuremath{{\mathcal V}}\xspace}
\newcommand{\cW}{\ensuremath{{\mathcal W}}\xspace}
\newcommand{\cX}{\ensuremath{{\mathcal X}}\xspace}
\newcommand{\cY}{\ensuremath{{\mathcal Y}}\xspace}
\newcommand{\cZ}{\ensuremath{{\mathcal Z}}\xspace}


==> src/table/kemeny.tex <==
\begin{table}[htbp]
    \tabcolsep=1.6pt
    \centering
    %\footnotesize
    \fontsize{7.5}{8.2}\selectfont
    \begin{threeparttable}
        \caption{Experimental results on model network $\mathcal{F}'_{g}$ with various $g$. We report exact $K(\mathcal{F}'_g)$ as well as its approximations $\tilde{K}(\mathcal{F}'_g)$ and $\hat{K}(\mathcal{F}'_g)$, relative errors $\rho_1=|K(\mathcal{F}'_g)-\tilde{K}(\mathcal{F}'_g)|/K(\mathcal{F}'_g)$ and $\rho_2=|K(\mathcal{F}'_g)-\hat{K}(\mathcal{F}'_g)|/K(\mathcal{F}'_g)$, and running times (seconds, $s$) $s_1$ for computing $\tilde{K}(\mathcal{F}'_g)$ and $s_2$ for computing $\hat{K}(\mathcal{F}'_g)$. $K(\mathcal{F}'_g)$ is obtained via equation~\eqref{Kemeny04}, $\tilde{K}(\mathcal{F}'_g)$ and $\hat{K}(\mathcal{F}'_g)$ are obtained through \textsc{ApproxDelta} and \textsc{SampleDelta} with $\epsilon=0.3$, respectively.}
        \label{tab:Kemeny}
        \begin{tabular}{cccccccc}
            \toprule
            Network             & $K(\mathcal{F}'_g)$ & $\tilde{K}(\mathcal{F}'_g)$ & $\hat{K}(\mathcal{F}'_g)$ & $\rho_1$ & $\rho_2$ & $s_1$    & $s_2$\cr
            \midrule
            %\specialrule{0em}{3pt}{3pt}
            %$\mathcal{F}'_{10}$              & 127,285 & 129,884 & 125,010 & 0.020 & 0.017 & 64.554 & 6.801\cr
            %\specialrule{0em}{3pt}{3pt}
            %$\mathcal{F}'_{11}$              & 382,706 & 389,865 & 377,644 & 0.018 & 0.013 & 208.048 & 39.173 \cr
            \specialrule{0em}{3pt}{3pt}
            $\mathcal{F}'_{12}$ & 1,149,823           & 1,171,556                   & 1,130,961                 & 0.018    & 0.016    & 740.758  & 72.870\cr
            \specialrule{0em}{3pt}{3pt}
            $\mathcal{F}'_{13}$ & 3,452,880           & 3,519,052                   & 3,389,888                 & 0.019    & 0.018    & 3465.607 & 135.735\cr
            \specialrule{0em}{3pt}{3pt}
            $\mathcal{F}'_{14}$ & 1.036$\times 10^7$  &                             & 1.018$\times 10^7$        &          & 0.017    &          & 230.798  \cr
            \specialrule{0em}{3pt}{3pt}
            $\mathcal{F}'_{15}$ & 3.111$\times 10^7$  &                             & 3.051$\times 10^7$        &          & 0.019    &          & 476.335  \cr
            \specialrule{0em}{3pt}{3pt}
            \bottomrule
        \end{tabular}
        %	\begin{tablenotes}
        %\end{tablenotes}
    \end{threeparttable}
\end{table}


==> src/table/kemeny_old.tex <==
\begin{table}[htbp]
    \tabcolsep=3pt
    \centering
    %\footnotesize
    \fontsize{7.9}{8.5}\selectfont
    \begin{threeparttable}
        \caption{Experimental results on model network $\mathcal{F}'_{g}$. We report the exact $K(\mathcal{F}'_g)$, its approximation $\tilde{K}(\mathcal{F}'_g)$, relative error $\rho=|K(\mathcal{F}'_g)-\tilde{K}(\mathcal{F}'_g)|/K(\mathcal{F}'_g)$, and running time (seconds, $s$) for computing $\tilde{K}(\mathcal{F}'_g)$, where
        $K(\mathcal{F}'_g)$ is obtained via~\eqref{Kemeny04} and $\tilde{K}(\mathcal{F}'_g)$ is obtained through \textsc{ApproxDelta} with $\epsilon=0.3$.}
        \label{tab:Kemeny}
        \begin{tabular}{ccccccc}
            \toprule
            Network             & Nodes (\#) & Edges (\#) & $K(\mathcal{F}'_g)$ & $\tilde{K}(\mathcal{F}'_g)$ & Error $\rho$ & Time\cr
            \midrule
            \specialrule{0em}{3pt}{3pt}
            $\mathcal{F}'_{10}$ & 88,575     & 177,147    & 127,285             & 129,884                     & 0.020        & 64.554\cr
            \specialrule{0em}{3pt}{3pt}
            $\mathcal{F}'_{11}$ & 265,722    & 531,441    & 382,706             & 389,865                     & 0.018        & 208.048\cr
            \specialrule{0em}{3pt}{3pt}
            $\mathcal{F}'_{12}$ & 797,163    & 1,594,323  & 1,149,823           & 1,171,556                   & 0.018        & 740.758\cr
            \specialrule{0em}{3pt}{3pt}
            $\mathcal{F}'_{13}$ & 2,391,486  & 4,782,969  & 3,452,880           & 3,519,052                   & 0.019        & 3465.607\cr
            \specialrule{0em}{3pt}{3pt}
            \bottomrule
        \end{tabular}
        %	\begin{tablenotes}
        %\end{tablenotes}
    \end{threeparttable}
\end{table}

==> src/table/large_disagree.tex <==
\begin{table}[!b]
    \centering
    \tabcolsep=2pt
    \fontsize{7.5}{8.3}\selectfont
    \begin{threeparttable}
        \caption{Statistics and results for large connected real networks. For each network, we indicate the number of nodes $N$, the number of edges $M$, running time (seconds, $s$) $s_1$ and $s_2$ for \textsc{ApproxDelta} and \textsc{SampleDelta}, approximations $\tilde{\delta}$ and $\hat{\delta}$ of opinion disagreement computed by \textsc{ApproxDelta} and \textsc{SampleDelta}.}
        \label{tab:large_disagree}
        \begin{tabularx}{8cm}{ccccccc}
            \Xhline{2\arrayrulewidth}
            %\specialrule{0em}{1.5pt}{1pt}
            Network                             & $N$        & $M$        & $s_1$    & $s_2$    & $\tilde{\delta}$ & $\hat{\delta}$ \cr
            \midrule
            %soc-livemocha   & 104,103 & 2,193,083 & 3517.567  & 48.285  & 1.028 & 0.994 \cr
            %lex-wordnet            & 146,005 & 656,999 & 145,145 & 656,230 \cr
            %soc-douban & 154,908 & 327,162 &289.951  & 35.562  &1.595 & 1.587  \cr
            %soc-gowalla & 196,591 & 950,327 &807.861 & 237.41 &1.199 & 1.205\cr
            %ca-DBLP & 317,080 & 1,049,866 &681.720& 124.132 & 1.519  &  1.484\cr
            %misc-amazon & 334,863 & 925,872 &539.675& 143.277 & 2.185 & 1.952 \cr
            {\footnotesize soc-twitter-follows} & 404,719    & 713,319    & 1149.346 & 342.315  & 2.377            & 2.399 \cr
            soc-delicious                       & 536,108    & 1,365,961  & 1717.988 & 433.302  & 1.691            & 1.624 \cr
            %inf-pennsylvania       & 1,088,092 & 1,541,898 & 1,087,562 & 1,541,514 \cr
            {\footnotesize soc-youtube-snap}    & 1,134,890  & 2,987,624  & 7411.479 & 163.753  & 1.581            & 1.504\cr
            %roadNet-TX         & 1,379,917 & 1,921,660 & 1,351,137 & 1,879,201 \cr
            soc-hyves                           & 1,402,673  & 2,777,419  & 5823.603 & 184.275  & 1.671            & 1.660\cr
            delaunay-n24                        & 16,777,216 & 50,331,601 &          & 129.777  &                  & 1.698\cr
            road-usa                            & 23,947,347 & 28,854,312 &          & 133.549  &                  & 4.891\cr
            socfb-konect                        & 58,790,782 & 92,208,195 &          & 3856.067 &                  & 2.257\cr
            \Xhline{2\arrayrulewidth}
        \end{tabularx}
    \end{threeparttable}
\end{table}


==> src/table/notations.tex <==
\begin{table}[htbp]
    \centering
    \caption{Frequently used notations.}
    \label{tab:notation}
    \begin{tabularx}{\linewidth}{rX}
        \toprule
        \textbf{Notation} & \textbf{Description}                                    \\
        \midrule
        \(\G=(\V,\E,w)\)  & A connected undirected weighted network.                \\
        \(\PP\)           & The transition matrix of random walks on \(\G\).        \\
        \(\G'\)           & The weighted graph with transition matrix \(\PP^2\).    \\
        \(\tilde{\G}\)    & The sparsified graph of \(\G'\) by Lemma~\ref{eq:Ltil}. \\
         \(\bar{\G}\)    & The graph obtained from  \(\tilde{\G}\) by deleting loops. \\
        \bottomrule
    \end{tabularx}
\end{table}


==> src/table/real_disagree.tex <==
\begin{table}[t]
    \centering
    \normalsize
    \tabcolsep=3pt
    \fontsize{7}{8}\selectfont
    \begin{threeparttable}
        \caption{Statistics and experimental results for some real-world networks. We indicate both node number $N$ and edge number $M$ of LCC, power-law exponent $\gamma$, opinion disagreement $\delta$ computed by the exact algorithm (Exact) through~\eqref{eq:delta02}, the approximation $\tilde{\delta}$ of $\delta$ computed by Algorithm~\ref{alg:approx_delta} \textsc{ApproxDelta}, the approximation $\hat{\delta}$ of $\delta$ computed by Algorithm~\ref{alg:sample_delta} \textsc{SampleDelta}, relative error $\rho_1=|\delta-\tilde{\delta}|/\delta$, and relative error $\rho_2=|\delta-\hat{\delta}|/\delta$.
        }
        \label{tab:real_disagree}
        \begin{tabular}{ccccccccc}
            \toprule
            \multirow{3}{*}{Network} & \multirow{3}{*}{$N$} & \multirow{3}{*}{$M$} & \multirow{3}{*}{$\gamma$} &
            \multicolumn{5}{c}{Opinion Disagreement}\cr
            \cmidrule{5-9}
                                     &                      &                      &                           & $\delta$ & $\tilde{\delta}$ & $\hat{\delta}$ & $\rho_1$ & $\rho_2$ \cr
            \midrule
            %\multicolumn{12}{c}{\textbf{Biological Networks}}\cr
            %%%
            {Zachary}                & {34}                 & {78}                 & {2.161}                   & 1.287    & 1.300            & 1.294          & 0.010    & 0.005  \cr
            bio-celegans             & 453                  & 2,025                & 2.621                     & 1.132    & 1.028            & 1.187          & 0.017    & 0.049 \cr
            {web-polblogs}           & {643}                & {2,280}              & {2.021}                   & 1.300    & 1.300            & 1.299          & 0.000    & 0.001 \cr
            %{U. Rovira i Virgili}&  {1,133} &  {5,451} &  {1.561} &  1.149 & 1.154 & 1.147 & 0.004 & 0.002 \cr
            {Protein}                & {1,458}              & {1,948}              & {2.879}                   & 3.081    & 3.205            & 3.046          & 0.040    & 0.011\cr
            {soc-hamsterster}        & {2,000}              & {16,097}             & {2.421}                   & 1.140    & 1.146            & 1.137          & 0.005    & 0.003\cr
            {socfb-Amherst41}        & {2,235}              & {90,954}             & {2.361}                   & 1.013    & 1.017            & 1.013          & 0.004    & 0.000 \cr
            {Human protein (Vidal)}  & {2,783}              & {6,007}              & {2.132}                   & 1.515    & 1.530            & 1.517          & 0.010    & 0.001 \cr
            %{web-edu}  &  {3,031} &  {6,474} &  {2.161} &  5.904 & 5.885 & 4.439 & 0.003 & 0.248\cr
            %%%
            {bio-grid-worm}          & {3,343}              & {6,437}              & {2.161}                   & 1.681    & 1.681            & 1.674          & 0.000    & 0.004  \cr
            {socfb-Mich67}           & {3,745}              & {81,901}             & {2.521}                   & 1.025    & 1.031            & 1.027          & 0.005    & 0.002  \cr
            {soc-PagesTVshow}        & {3,892}              & {17,239}             & {2.740}                   & 1.766    & 1.801            & 1.698          & 0.020    & 0.039  \cr
            %	{ca-GrQc} &  {4,158} &  {13,422} &  {2.061} & 2.249 & 2.293 & 1.840 & 0.019 & 0.182 \cr
            {web-EPA}                & {4,253}              & {8,897}              & {2.461}                   & 1.791    & 1.787            & 1.785          & 0.002    & 0.003 \cr
            {web-spam}               & {4,767}              & {37,375}             & {2.381}                   & 1.126    & 1.129            & 1.124          & 0.002    & 0.002 \cr

            % {ca-Erdos992} &  {5,094} &  {7,515} &  {4,991} &  {7,428} &  {2.181} &  {2.401}  \cr
            %			{Reactome}  &  {5,973} &  {145,778} &  {1.363} &1.115 & 1.114 & 1.107 & 0.001 & 0.007 \cr
            {socfb-American75}       & {6,370}              & {217,654}            & {2.441}                   & 1.016    & 1.018            & 1.016          & 0.001    & 0.000 \cr
            {socfb-MIT}              & {6,402}              & {251,230}            & {2.221}                   & 1.013    & 1.016            & 1.013          & 0.002    & 0.000 \cr
            {Routeviews}             & {6,474}              & {12,572}             & {2.462}                   & 1.617    & 1.633            & 1.620          & 0.009    & 0.002  \cr
            {socfb-CMU}              & {6,621}              & {249,959}            & {2.301}                   & 1.014    & 1.019            & 1.014          & 0.004    & 0.000\cr
            {soc-PagesGovernment}    & {7,057}              & {89,429}             & {2.751}                   & 1.082    & 1.082            & 1.081          & 0.000    & 0.001 \cr

            %\midrule
            %\multicolumn{12}{c}{\textbf{Collaboration Networks}}\cr
            {socfb-Duke14}           & {9,885}              & {506,437}            & {2.061}                   & 1.010    & 1.012            & 1.011          & 0.001    & 0.001\cr
            {socfb-Bingham82}        & {10,001}             & {362,892}            & {2.421}                   & 1.015    & 1.015            & 1.015          & 0.000    & 0.000 \cr


            {ca-HepPh}               & {11,204}             & {117,619}            & {2.081}                   & 1.177    & 1.192            & 1.152          & 0.012    & 0.021  \cr
            {socfb-Stanford3}        & {11,586}             & {568,309}            & {2.001}                   & 1.011    & 1.012            & 1.011          & 0.001    & 0.000 \cr
            {socfb-Baylor93}         & {12,799}             & {679,815}            & {2.061}                   & 1.010    & 1.010            & 1.010          & 0.000    & 0.000 \cr
            %{soc-PagesCompany}&  {14,113} &  {52,126} &  {3.410} &  1.387 & 1.406 & 0.01\cr

            {ca-AstroPh}             & {17,903}             & {196,972}            & {2.861}                   & 1.096    & 1.096            & 1.096          & 0.000    & 0.000  \cr
            %\midrule
            %\multicolumn{12}{c}{\textbf{Social Networks}}\cr
            {soc-Gplus}              & {23,613}             & {39,182}             & {2.621}                   & 3.654    & 3.720            & 3.567          & 0.018    & 0.024 \cr
            {CAIDA}                  & {26,475}             & {53,381}             & {2.509}                   & 1.607    & 1.624            & 1.622          & 0.010    & 0.009\cr
            %{soc-GemsecRO}&  {41,773} &  {125,826} &  {4.380} &   1.304 & 1.318 & 0.010 \cr
            %{soc-GemsecHU} &  {47,538} &  {222,887} &  {4.940} &   1.152 & 1.159 & 0.005 \cr
            {soc-PagesArtist}        & {50,515}             & {819,090}            & {2.261}                   & 1.038    & 1.040            & 1.038          & 0.002    & 0.000  \cr
            {Brightkite}             & {56,739}             & {212,945}            & {2.481}                   & 1.269    & 1.278            & 1.265          & 0.007    & 0.003  \cr
            %\midrule
            %\multicolumn{12}{c}{\textbf{Web Networks}}\cr


            \Xhline{2\arrayrulewidth}
        \end{tabular}
    \end{threeparttable}
\end{table}

